MulSMo: Multimodal Stylized Motion Generation by Bidirectional Control Flow

Generating motion sequences conforming to a target style while adhering to the given content prompts requires accommodating both the content and style. In existing methods, the information usually only flows from style to content, which may cause conflict between the style and content, harming the integration. Differently, in this work we build a bidirectional control flow between the style and the content, also adjusting the style towards the content, in which case the style-content collision is alleviated and the dynamics of the style is better preserved in the integration. Moreover, we extend the stylized motion generation from one modality, i.e. the style motion, to multiple modalities including texts and images through contrastive learning, leading to flexible style control on the motion generation. Extensive experiments demonstrate that our method significantly outperforms previous methods across different datasets, while also enabling multimodal signals control. The code of our method will be made publicly available.

==> algorithm/100STYLE_Label.tex <==
% \usepackage{tabularx} % 在导言区加载 tabularx 包

\begin{table*}[h]
\centering
\label{tab:100style}
\begin{tabularx}{\textwidth}{|c|X|}
\hline
\textbf{Category} & \textbf{Label} \\ \hline
CHAR & Aeroplane, Cat, Chicken, Dinosaur, Fairy, Monk, Morris, Penguin, Quail, Roadrunner, Robot, Rocket, Star, Superman, Zombie (15) \\ \hline
PER & Balance, Heavyset, Old, Rushed, Stiff (5) \\ \hline
EMO & Angry, Depressed, Elated, Proud (4) \\ \hline
ACT & kimbo, ArmsAboveHead, ArmsBehindBack, ArmsBySide, ArmsFolded, BeatChest, BentForward, BentKnees, BigSteps, BouncyLeft, BouncyRight, CrossOver, FlickLegs, Followed, GracefulArms, HandsBetweenLegs, HandsInPockets, HighKnees, KarateChop, Kick, LeanBack, LeanLeft, LeanRight, LeftHop, LegsApart, LimpLeft, LimpRight, LookUp, Lunge, March, Punch, RaisedLeftArm, RaisedRightArm, RightHop, Skip, SlideFeet, SpinAntiClock, SpinClock, StartStop, Strutting, Sweep, Teapot, Tiptoe, TogetherStep, TwoFootJump, WalkingStickLeft, WalkingStickRight, Waving, WhirlArms, WideLegs, WiggleHips, WildArms, WildLegs (58) \\ \hline
MOT & CrowdAvoidance, InTheDark, LawnMower, OnHeels, OnPhoneLeft, OnPhoneRight, OnToesBentForward, OnToesCrouched, Rushed (9) \\ \hline
OBJ & DragLeftLeg, DragRightLeg, DuckFoot, Flapping, ShieldedLeft, ShieldedRight, Swimming, SwingArmsRound, SwingShoulders (9)\\ \hline
\end{tabularx}
\caption{The detailed grouping of style labels in the 100STYLE dataset.}
\end{table*}


==> sections/0_teaser.tex <==

\let\oldtwocolumn\twocolumn
\renewcommand\twocolumn[1][]{%
    \oldtwocolumn[{#1}{
    \begin{center}
           \includegraphics[width=\textwidth]{figures/teaser_2col.pdf}
           % \vspace{2.7in}
           \captionof{figure}{\textbf{MulSMo} enables flexible style signals to control the stylized motion generation, including motion sequences, texts, and images.}
            \label{fig:teaser}
        \end{center}
    }]
}
